Sample Complexity of Distributionally Robust Average-Reward Reinforcement Learning

Motivated by practical applications where stable long-term performance is critical-such as robotics, operations research, and healthcare-we study the problem of distributionally robust (DR) average-reward reinforcement learning. We propose two algorithms that achieve near-optimal sample complexity. The first reduces the problem to a DR discounted Markov decision process (MDP), while the second, Anchored DR Average-Reward MDP, introduces an anchoring state to stabilize the controlled transition kernels within the uncertainty set. Assuming the nominal MDP is uniformly ergodic, we prove that both algorithms attain a sample complexity of $\widetilde{O}\left(|\mathbf{S}||\mathbf{A}| t_{\mathrm{mix}}^2\varepsilon^{-2}\right)$ for estimating the optimal policy as well as the robust average reward under KL and $f_k$-divergence-based uncertainty sets, provided the uncertainty radius is sufficiently small. Here, $\varepsilon$ is the target accuracy, $|\mathbf{S}|$ and $|\mathbf{A}|$ denote the sizes of the state and action spaces, and $t_{\mathrm{mix}}$ is the mixing time of the nominal MDP. This represents the first finite-sample convergence guarantee for DR average-reward reinforcement learning. We further validate the convergence rates of our algorithms through numerical experiments.

==> sections/04Extension.tex <==
\section{Extenstion to \texorpdfstring{$f_k$-divergence}{f-divergence} family}
\label{sec:extenstion_to_f_divergence_family}

We extend the analysis of the Algorithm \ref{alg:reduction_to_dmdp}, \ref{alg:anchored_amdp} to the setting is constrained to perturbations with Cressie-Read family of $f_k$-divergence balls of radius $\delta$. The $f$-divergence which is parameterized by $(1, \infty)$. 
While our results could be generalized to other values of $k$, we focus on the value range $k\in (1, \infty)$, define:
\begin{equation}
    f_k(t) := \frac{t^k - kt + k-1}{k(k-1)}
\end{equation}
The Cressie-Read famility $f_k$-divergence parameterized by $k$ is defined as:
\begin{equation}
    D_{f_k}\bracket{Q\|P} := \int_{\Omega}f_k\bracket{\frac{dQ}{dP}}P(d\omega)
\end{equation}
Note that the $\chi^2$ divergence is the $f_k$-divergence with $k=2$. The Cressie-Read $f_k$-divergence and KL-divergence do not contain each other and are complementary.

We reuse the notation for the KL-divergence case in the discussion of this section. For each $(s,a)\in \Ss\times \Aa$ and $\delta > 0$, we define the $f_k$-divergence sets as:
\begin{align}
    \label{equ:fk_uncertainty_set}
    \calP_{s,a}(D_{f_k}, \delta) &:= \set{p: D_{f_k}(p\|p_{s,a})\leq \delta} & \calP(D_{f_k}, \delta) = & \bigtimes_{(s,a)\in \Ss\times \Aa}\calP_{s,a}(\delta)
\end{align}
For $f_k$-divergence defined in \eqref{equ:fk_uncertainty_set}, the dual functional can be found as:
\begin{lemma}[Lemma 1 of \cite{duchi_learning_2020}]
    For any $(s,a)\in \Ss \times \Aa$, let $\calP_{s,a}$ be the $f_k$-uncertainty set centered at the nominal transition kernel $p_{s,a}$. Then, for any $\delta > 0$, let $k^* = \frac{k}{k-1}$:
    \begin{equation}
        \Gamma_{\calP_{s,a}}(V) = \sup_{\alpha \in \R}\set{\alpha - c_k(\delta) E_{p_{s,a}}\left[\left(\alpha - V(S)\right)_+^{k^*}\right]^{\frac{1}{k^*}}}
    \end{equation}
    where $c_k(\delta) = \bracket{1 + k(k-1)\delta}^{\frac{1}{k}}$, $(\cdot)_+ = \max\set{\cdot, 0}$ and $V:\Ss \to \R$ is the value function.
\end{lemma}
\todo[color=red]{Zijun:Do I need to move the fk-dual functional into the appendix, as the body part length is limited lol...}

Recall the definition of the minimal support probability $\essinfp$ in \ref{defn:minimal_support_probability}. Similar in the KL-divergence case, we consider the the regime with limited adversarial Power:
\begin{assumption}[Limited Adversarial Power]
\label{ass:limited_adversarial_power_fk_divergence}
    For $f_k$-divergence, we assume the the uncertainty size $\delta$ satisfies: $\delta \leq \frac{1}{4\max\set{2,k}\maxm^2}\essinfp$
\end{assumption}

\begin{theorem}
    \label{thm:sample_complexity_for_reduction_to_dmdp_fk_divergence}
    Suppose Assumptions \ref{ass:bounded_minorization_time}, \ref{ass:limited_adversarial_power_fk_divergence} are in force. Then, for any $n\geq \frac{32\maxm^2}{\essinfp}\log\frac{2|S|^2|A|}{\beta}$ and $\varepsilon > 0$, the policy $\widehat \pi^*$ and $g_{\hatP}^*$ returned by Algorithm \ref{alg:reduction_to_dmdp} satisifes:
    \begin{equation}
    	\begin{aligned}
    		0\leq g_\calP^* - g_\calP^{\widehat\pi^*}\leq& 120\tmin\sqrt{\frac{2}{n\essinfp}\log\frac{2|\Ss|^2|\Aa|}{\beta}}\\
    		\linftynorm{g_{\hatP}^* - g_{\calP}^*}\leq & 60\tmin\sqrt{\frac{2}{n\essinfp}\log\frac{2|\Ss|^2|\Aa|}{\beta}}
    	\end{aligned}
    \end{equation}
    with probability $1-\beta$, and the sample complexity to achieve $\varepsilon$-optimal policy and value function with probability $1-\beta$ is:
    \[
    n\leq \frac{c\cdot \tmin^2}{\essinfp \varepsilon^2}\log\frac{2|S|^2|A|}{\beta}
    \]
\end{theorem}
\begin{corollary}
	\label{cor:sample_complexity_for_anchored_amdp_fk_divergence}
	Following the setting of Theorem \ref{thm:sample_complexity_for_reduction_to_dmdp_fk_divergence}, the policy $\widehat\pi^*$ and $g_{\underline{\hatP}}^*$ returned by Algorithm \ref{alg:anchored_amdp} satisifes:
	\begin{equation}
		\begin{aligned}
			0\leq g_{\calP}^* - g_{\calP}^{\widehat\pi^*} \leq& 120\tmin\sqrt{\frac{2}{n\essinfp}\log\frac{2|\Ss|^2|\Aa|}{\beta}}\\
			\linftynorm{g_{\underline{\hatP}}^* - g_{\calP}^*}\leq & 60\tmin\sqrt{\frac{2}{n\essinfp}\log\frac{2|\Ss||\Aa|}{\beta}}
		\end{aligned}
	\end{equation}
	with probability $1-\beta$, and the sample complexity to achieve $\varepsilon$-optimal policy and value function with probability $1-\beta$ is:
	\[
	n\leq\frac{c\cdot \tmin^2}{\essinfp \varepsilon^2}\log\frac{2|\Ss|^2|\Aa|}{\beta}
	\]
\end{corollary}
The proof of Theorem \ref{thm:sample_complexity_for_reduction_to_dmdp_fk_divergence} closely follows the proof of Theorem \ref{thm:sample_complexity_for_reduction_to_dmdp}. We first analysis the Radon-Nikodym derivative and minorization time over uncertainty set $\calP$ for $f_k$-divergence uncertainty set case. The sample complexity is then derived by aggregating the analysis in similar with Theorem \ref{thm:sample_complexity_for_reduction_to_dmdp}. This procedure is carried out in Appendix.
